Planning of Power Grasps Using Infinite Program Under Complementary Constraints

We propose an optimization-based approach to plan power grasps. Central to our method is a reformulation of grasp planning as an infinite program under complementary constraints (IPCC), which allows contacts to happen between arbitrary pairs of points on the object and the robot gripper. We show that IPCC can be reduced to a conventional finite-dimensional nonlinear program (NLP) using a kernel-integral relaxation. Moreover, the values and Jacobian matrices of the kernel-integral can be evaluated efficiently using a modified Fast Multipole Method (FMM). We further guarantee that the planned grasps are collision-free using primal barrier penalties. We demonstrate the effectiveness, robustness, and efficiency of our grasp planner on a row of challenging 3D objects and high-DOF grippers, such as Barrett Hand and Shadow Hand, where our method achieves superior grasp qualities over competitors.

==> ref/Q_metric_old.tex <==
\section{Epsilon-Subdifferential of Grasp Metric}
In \prettyref{eq:strict}, we derived the softened version of the collision-free guarantee. This section, we augment the formulation to derive a complete optimization-based grasp planner. An optimization-based grasp planner requires some metric that measures the quality of a grasp. Let's assume that we use a $Q_1$ metric, which is defined as follows:
\begin{equation}
\label{eq:Q}
Q_1=\fmax{\E{f_i}}r\quad \ST \{\E{w}|\|\mathbb{M}\textbf{w}\|\leq r\} \subseteq{\mathbb{W}}\\
\end{equation}
\begin{align*}
\mathbb{W} = \left\{ \sum_i 
    \begin{pmatrix}
    \textbf{f}_i \\ \textbf{p}_i \times \textbf{f}_i
    \end{pmatrix} \bigg\rvert
    \begin{pmatrix}
    \sum_i \textbf{f}_i^T \textbf{n}(\textbf{p}_i) \leq 1\\ 
    \|\textbf{f}_i - \textbf{n}(\textbf{p}_i)\textbf{n}(\textbf{p}_i)^\textit{T} \|_2 \leq \mu\textbf{f}_i^T\textbf{n}(\textbf{p}_i)
    \end{pmatrix}\right\}\\
\end{align*}
where $\mu$ is the frictional coefficient and $\mathbb{M}$ is a user-provided tensor $\textbf{Diag}(1,1,1,m,m,m)$. More specifically, $Q_1$ can be treated as the radius of the origin-centered 6D sphere in the admissible wrench space, in which wrenches should be confined by two conditions: limited force magnitude and friction cone constraints.\\
In prior work \cite{Liu2020DeepDG}, the first condition for feasible wrenches at inexact potential contact points $\textbf{p}_i$ is modified to a differentiable form with an exponential decay:
\begin{equation}
    \sum_{i} \mathbf{f}_{i}^{T} \mathbf{n}\left(\mathbf{p}_{i}\right) \textbf{exp} \left(\alpha\left\|\mathbf{d}\left(\mathbf{p}_{i}\right)\right\|%+\beta\left(1+\mathbf{n}\left(\mathbf{p}_{i}\right)^{T} \mathbf{n}_{g}\left(\mathbf{p}_{i}\right)\right)
    \right) \leq 1
\end{equation}
which takes the distance between the robot hand and the target object $\textbf{d}(\textbf{p}_i)$ into consideration, namely, allowing the robot hand and the target object are not strictly in contact. In addition to this modification, the traditional $Q_1$ is extended to a generalized $Q_1$ metric  under the assumption that $\textbf{w}$ must be along one of a discrete set of directions: $\textbf{s}_{1,\cdots,\textit{\textbf{D}}}$ as follows:
\begin{align}
    \label{eq:directional Q}
    Q_{1}&=\fmin{j=1, \cdots, D}\left[\fmax{\mathbf{w} \in \mathbb{W}} \mathbf{s}_{j}^{T} \mathbb{M} \mathbf{w}\right] \nonumber\\
    &=\fmin{j=1, \cdots, D} \left[\fmax{i=1, \cdots, N} \fmax{\mathbf{w} \in \mathbb{W}_{i}} \mathbf{s}_{j}^{T} \mathbb{M}\mathbf{w}\right]
\end{align}
where\\ 
\begin{equation*}
\mathbb{W}_{i} \triangleq\left\{
    \begin{pmatrix}
        \textbf{f}_i \\ \textbf{p}_i \times \textbf{f}_i
    \end{pmatrix} \bigg\rvert 
    \begin{pmatrix}
        \mathbf{f}_{i}^{T} \mathbf{n}\left(\mathbf{p}_{i}\right) \leq \textbf{exp} \left(-\alpha\left\|\mathbf{d}\left(\mathbf{p}_{i}\right)\right\| \right) \\ \left\|\mathbf{f}_{i}-\mathbf{n}\left(\mathbf{p}_{i}\right) \mathbf{n}\left(\mathbf{p}_{i}\right)^{T} \mathbf{f}_{i}\right\|_{2} \leq \mu\mathbf{f}_{i}^{T} \mathbf{n}\left(\mathbf{p}_{i}\right) 
    \end{pmatrix}\right\}
\end{equation*}
In our work, we are assuming that the robot hand and the target object are convex hulls and the shapes that are not convex will be decomposed into convex hulls. Consequently, there are no sampled potential contact points $\textbf{p}_i$ on the robot hand. Instead, for each pair of convex shapes of the hand and the target, we define $\textbf{n}_{ab}^{(i)}$ and $d_{ab}^{(i)}$ for them as in section \RN{3}. Therefore, the distance was no longer $\textbf{d}(\textbf{p}_i)$ but $\textbf{dist}_{ab}^{(i)}$.
\\According to the new formulation, new admissible wrench space becomes:
\begin{equation*}
\mathbb{W}_{i} \triangleq\left\{
    \begin{pmatrix}
        \textbf{f}_{ab}^{(i)} \\ \textbf{p}_{ab}^{(i)} \times \textbf{f}_{ab}^{(i)}
    \end{pmatrix} \bigg\rvert 
    \begin{pmatrix}
        {\mathbf{f}_{ab}^{(i)}}^{T} \mathbf{n}_{ab}^{(i)} \leq \textbf{exp} \left(-\alpha\left\|\mathbf{dist}_{ab}^{(i)}\right\|\right) \\ \left\|\mathbf{f}_{ab}^{(i)}-\mathbf{n}_{ab}^{(i)} \mathbf{n}_{ab}^{(i)} \mathbf{f}_{ab}^{(i)}\right\|_{2} \leq \mu{\mathbf{f}_{ab}^{(i)}}^{T} \mathbf{n}_{ab}^{(i)} 
    \end{pmatrix}\right\}
\end{equation*}
\subsection{Wrench Space Analysis for $Q_1$ metric}
As described above, $Q_1$ metric is a rather intricate composite function with multiple levels. Thus, we will analyze it from the bottom level to the top. 
\subsubsection{Calculation of $\textbf{dist}_{ab}^{(i)}$}
$\textbf{dist}_{ab}^{(i)}$ is the distance between the robot hand and the target object. Based on the assumption that all target objects and the robot hand are convex decomposed into different convex shapes, determining the distance becomes the following QP programming problem aiming to solve the smallest distance between a pair of convex shapes:
\begin{align*}
   \textbf{dist}_{ab}^{(i)} = \fmin{\textbf{x}_1,\textbf{x}_2}
   \left\| \textbf{x}_1 - \textbf{x}_2 \right\|_2 \quad
    \ST \textbf{x}_1 \in \textbf{C}_a^{(i)},
              \textbf{x}_2 \in \textbf{C}_b^{(i)}
\end{align*}
However, for the simplicity of calculation and differentiability of the distance function, the distance between the centroids of two convex shapes could be an alternative choice for the QP solution as follows:
\begin{equation}
    \textbf{dist}_{ab}^{(i)} =\left\| \textbf{Centroid}_a^{(i)} - \textbf{Centroid}_b^{(i)} \right\|_2 \\
\end{equation}
\subsubsection{Exponential Decay}
Our exponential decay is the key to the differentiability of the first condition in the admissible wrench space even when the robot hand are not strictly touching the target. Specially, we define the exponential decay as follow:
\begin{equation}
    \textbf{ED} = \textbf{exp}\left(-\alpha\left\|\textbf{dist}_{ab}^{(i)} \right\|\right)
\end{equation}
In fact, $\textbf{ED}$ not only allows the differentiability for the first condition, but also defines a reasonable upper bound for $\textbf{f}_{ab}^{(i)}$ in the $\textbf{n}_{ab}^{(i)}$ direction, namely, the upper bound for the support force.\\
\subsubsection{Calulation of $Q_1$}

\subsection{Optimization Based Grasp Planner}
As shown in section \RN{3}, our log-barrier tunneling-free guarantee prevents the penetration between the robot hand and the target object from happening, but the side effect is that the robot hand could be repelled from the target as the log-barrier's driven it. As a result, we still need a reasonable objective function to ensure that at the final stage the robot hand would converge to a qualified pose and neutralize the side effect of log-barriers. Here, we propose $Q_1$ metric to be this objective function since it takes both grasp quality and distance into account. Thus, the best pose and position of the robot hand can be solved by following problem:
\begin{align}
\label{eq:Q1_optimization}
\argmax{\theta,\E{n}_{ab},d_{ab}}&\mathcal{Q}(\E{n}_{ab},d_{ab},\theta)\nonumber\\
   \mathcal{Q}(\E{n}_{ab},d_{ab},\theta) = \fmax{\theta,\textbf{n}_{ab}, d_{ab}} \left[ Q_1 \right. &+ \gamma \sum_{j=1}^{V(\E{C}_a)} \E{log} (\E{n}_{ab}^T \E{v}_a^j(\theta) - d_{ab})\nonumber\\ &+ \gamma \sum_{j=1}^{V(\E{C}_b)} \E{log}(d_{ab} - \E{n}_{ab}^T\E{v}_b^j(\theta)) \left.\right]
\end{align}
Since we have shown that $Q_1$ metric is a piece-wise linear function of $\textbf{ED}$, and non-differentiable at the boundary of each piece, directly optimizing \eqref{eq:Q1_optimization} using first-order gradient descent would be problematic. To solve \eqref{eq:Q1_optimization} properly, we introduce Gradient Sampling\cite{burke2020gradient} method to handle the non-differentiability of $Q_1$ metric. The algorithm is summarized in \prettyref{alg:gradient_sampling}:

\begin{algorithm}[ht]
\caption{Solve Objective function \eqref{eq:Q1_optimization}.}
\label{alg:gradient_sampling}
\begin{algorithmic}[1]
\Require{Initial guess for $\E{n}_{ab}^0,d_{ab}^0,\theta^0, \epsilon^0, \nu_0$.}
\For{Iteration $k=0,\cdots$}
\State Set $\beta^*\gets0,\phi^*\gets0$
\State Independently sample $\left\{ \theta^{k, 1}, \cdots, \theta^{k, m}  \right\}$  uniformly in $\mathbb{B}(\theta_k, \epsilon_k)$
\State compute $\mathcal{D}^{k}:=\operatorname{conv} \left\{\nabla \mathcal{Q}(\E{n}_{ab},d_{ab},\theta^{k}), \nabla \mathcal{Q}(\E{n}_{ab},d_{ab},\theta^{k,1}), \ldots, \nabla  \mathcal{Q}(\E{n}_{ab},d_{ab},\theta^{k,m})\right\}$.
\State \CMT{Either} Compute $\E{d}^{k}$ as the solution of $\min _{\E{d} \in \mathcal{D}^{k}} \frac{1}{2}\|\E{d}\|_{2}^{2}$
\State \CMT{Or} Compute search direction $\E{d}^k\triangleq\FPP{\left[\mathcal{Q}^k\right]^*}{\FOUR{\beta^*}{\phi^*}{d_{ab}^k}{\theta^k}}$
\If{$\left\|\E{d}^{k}\right\|_{2} \leq \nu_{\mathrm{opt}}$ and $\epsilon_{k} \leq \epsilon_{\mathrm{opt}}$} Terminate
\EndIf
\State Shrink $\nu_{k}$ by $\lambda_{\nu}$ Shrink $\epsilon_{k}$ by $\lambda_{\epsilon}$
\State Line search along $-\E{d}$ get $\alpha$
\State Set $\FOUR{\beta^{**}}{\phi^{**}}{d_{ab}^{k+1}}{\theta^{k+1}}=
\FOUR{\beta^*}{\phi^*}{d_{ab}^k}{\theta^k}-\alpha\E{d}^k$
\State Set $\E{n}_{ab}^{k+1}\gets\left[\E{n}_{ab}^k\right]^*(\beta^{**},\phi^{**})$
\EndFor
\end{algorithmic}
\end{algorithm}

==> ref/modelbased.tex <==
\section{Model-Based Learning}
When we optimize a grasping policy represented by a neural network, we further introduce a data loss:
\begin{align*}
\|\theta-\E{NN}(I,W)\|^2,
\end{align*}
and augment \prettyref{eq:SO} as a three-way optimization:
\begin{tiny}
\begin{align}
\label{eq:MSO}
\argmax{\substack{\AAA{\theta,\E{n}_{ab},d_{ab}}\\\BBB{Q,\E{f}_d^j},\CCC{W}}}&
\sum_{\substack{a=1,\cdots,M\\b=M+1,\cdots,M+N}}
\gamma\sum_{j=1}^{V(\E{C}_a)}\E{log}(\AAA{\E{n}_{ab}^T\E{v}_a^j(\theta)}-\AAA{d_{ab}})  \\
&+\sum_{\substack{a=1,\cdots,M\\b=M+1,\cdots,M+N}}
\gamma\sum_{j=1}^{V(\E{C}_b)}\E{log}(\AAA{d_{ab}}-\AAA{\E{n}_{ab}^T\E{v}_b^j(\theta)})+\BBB{Q}\nonumber \\
&-\|\AAA{\theta}-\E{NN}(I,\CCC{W})\|^2\nonumber   \\
\ST&\BBB{Q}\leq \sum_j{\E{s}^d}^T\BBB{\E{f}_{ab}}\quad\forall ab\nonumber   \\
&\AAA{\E{n}_{ab}^T}\BBB{\E{f}_{ab}}\leq\frac{\gamma}{\sum_{j=1}^{V(\E{C}_a)}(\AAA{\E{n}_{ab}^T\E{v}_a^j(\theta)}-\AAA{d_{ab}})+\sum_{j=1}^{V(\E{C}_b)}(\AAA{d_{ab}}-\AAA{\E{n}_{ab}^T\E{v}_b^j(\theta)})}\nonumber \\
&\mu\AAA{\E{n}_{ab}(\E{v}^j)^T}\BBB{\E{f}_d^j}\geq\|\left(\E{I}-\AAA{\E{n}_{ab}(\E{v}^j)\E{n}_{ab}(\E{v}^j)^T}\right)\BBB{\E{f}_d^j}\|.\nonumber
\end{align}
\end{tiny}
This optimization will be solved using a three-way ADMM. When we optimize $Q,\E{f}_d^j$, the problem is convex. When we optimize $\theta,\E{n}_{ab},d_{ab}$, the problem is non-convex, non-linear, solved using primal-only Newton-type method. When we optimize $W$, the problem becomes a supervised-learning, which is solved by mini-batch stochastic algorithm.

\subsection{Robust Model-Based Learning via Chamfer Loss}
A potential problem with \prettyref{eq:MSO} is that neural network only gets the chance to learn a single grasp pose per object, which is empirically too restrictive given a small architecture. To work around this, we use a similar idea as \cite{8968115} and replace the $l_2$-norm with a Chamfer loss, essentially allowing the neural network to pick which grasp pose it wants to represent. To formulate this, we rewrite \prettyref{eq:MSO} using the following shorthand notation:
\begin{align*}
\argmax{\substack{\AAA{\theta,\E{n}_{ab},d_{ab}}\\\BBB{Q,\E{f}_d^j},\CCC{W}}}&
\mathcal{O}(\AAA{\theta,\E{n}_{ab},d_{ab}},\BBB{Q,\E{f}_d^j})-\|\AAA{\theta}-\E{NN}(I,\CCC{W})\|^2,
\end{align*}
where the constraints are intact and we ignore them for brevity. Let's say that we allow the gripper to grasp an object from $V$ different views, where the depth image is: $I^{1,\cdots,V}$. For each view, we run an optimization from a different initial guess, so finally we will get $V$ different $\theta$. We use $\left[\bullet\right]_v$ to denote the index of each view. Then the Chamfer-loss takes the following form:
\begin{equation}
\begin{aligned}
\label{eq:CMSO}
\argmax{\substack{
\left[\AAA{\theta,\E{n}_{ab},d_{ab}}\right]_{1,\cdots,V}\\
\left[\BBB{Q,\E{f}_d^j},\CCC{W}\right]_{1,\cdots,V}}}&
\sum_{v=1}^V\mathcal{O}(\left[\AAA{\theta,\E{n}_{ab},d_{ab}},\BBB{Q,\E{f}_d^j}\right]_v)    \\
&-\fmin{v=1,\cdots,V}\|\left[\AAA{\theta}\right]_v-\E{NN}(I,\CCC{W})\|^2.
\end{aligned}
\end{equation}
This ultimate algorithm is outlined in \prettyref{alg:model_based}.
\begin{algorithm}[ht]
\caption{Solve \prettyref{eq:CMSO} \CMT{(Todo)}.}
\label{alg:model_based}
\begin{algorithmic}[1]
\For{Learning epoch $e=1,\cdots$}
\For{Each view $v=1,\cdots,V$}
\LineComment{Model-Based Search}
\State Find feasible initial guess $\left[\E{n}_{ab}^0,d_{ab}^0,\theta^0\right]_v$.
\For{Iteration $k=0,\cdots$}
\LineComment{Convex solver e.g. Mosek}
\State{Solve Eq\ref{eq:CMSO} ($\E{n}_{ab}^k,d_{ab}^k,\theta^k$) for $Q^k,\left[\E{f}_d^i\right]^k$}
\LineComment{Non-convex, primal-only solver}
\State{Solve Eq\ref{eq:CMSO} ($Q^k,\left[\E{f}_d^i\right]^k$) for $\E{n}_{ab}^{k+1},d_{ab}^{k+1},\theta^{k+1}$}
\If{$|Q^{k+1}-Q^k|<\epsilon$}
\State Record $\left[Q,\E{f}_d^i,\E{n}_{ab},d_{ab},\theta\right]_v$
\State Break
\EndIf
\EndFor
\EndFor
\LineComment{Supervised-Learning}
\State Update NN ($W$) by solving \prettyref{eq:CMSO} with SGD.
\EndFor
\end{algorithmic}
\end{algorithm}

==> ref/second_order.tex <==
\section{Second-Order Convergence}
In \prettyref{eq:strict}, we derived the softened version of the collision-free guarantee. This section, we augment the formulation to derive a complete optimization-based grasp planner, with twice-differentiable objectives and hard constraints. An optimization-based grasp planner requires some metric that measures the quality of a grasp. Let's assume that we use a $Q_\infty$ metric. Given a set of contact points $\{\E{v}^j\}$ on the gripper, and a set of sampled, 6D unit directions $\E{s}^{1,\cdots,D}$, we have shown in \cite{Liu2020DeepDG} that the tight upper bound of the $Q_\infty$ metric is the result of the following convex optimization:
\begin{small}
\begin{equation}
\begin{aligned}
\label{eq:Q}
&Q_\infty=\fmax{Q,\E{f}_{ab}}Q  \\
\ST&Q\leq \sum_j{\E{s}^d}^T\E{f}_{ab}\quad\forall ab   \\
&\E{n}_{ab}^T\E{f}_{ab}\leq1\nonumber \\
&\mu\E{n}_{ab}^T\E{f}_{ab}\geq\|\left(\E{I}-\E{n}_{ab}\E{n}_{ab}^T\right)\E{f}_{ab}\|,
\end{aligned}
\end{equation}
\end{small}
and the remaining problem is how do we combine the \prettyref{eq:strict} and \prettyref{eq:Q}. A major challenge is how do we define contact points: $\{\E{v}^j\}$. Since a contact point must be in touch with the object surface, we immediately have the following complementary constraint:
\begin{align*}
&0\leq
{\sum_{j=1}^{V(\E{C}_a)}(\E{n}_{ab}^T\E{v}_a^j(\theta)-d_{ab})+
\sum_{j=1}^{V(\E{C}_b)}(d_{ab}-\E{n}_{ab}^T\E{v}_b^j(\theta))}  \\
&\perp  \\
&0\leq\E{n}_{ab}\E{f}_{ab},
\end{align*}
where $\E{dist}(\E{v}^j)$ is distance from a point on the gripper to the object. However, we do not have a well-defined $\E{dist}(\E{v}^j)$ so far. Since we use dual convex-convex distance in \prettyref{eq:strict}, the distance is not explicitly defined. However, it is well-known that a log-barrier function such as $-\E{log}(d_{ab}-\E{n}_{ab}^T\E{v}_b^j(\theta))$ implicitly defines an approximated Lagrangian multiplier:
\begin{align*}
\lambda=\frac{\gamma}
{\sum_{j=1}^{V(\E{C}_a)}(\E{n}_{ab}^T\E{v}_a^j(\theta)-d_{ab})+
\sum_{j=1}^{V(\E{C}_b)}(d_{ab}-\E{n}_{ab}^T\E{v}_b^j(\theta))},
\end{align*}
which indicates the closeness between the gripper and the object. For a pair of convex shapes $\TWO{\E{C}_a}{\E{C}_b}$ where $\E{C}_a$ belongs to the gripper and $\E{C}_b$ belongs to the object, we propose to use the closeness indicator and relax the force-norm constraint as:
\begin{small}
\begin{align*}
\E{n}_{ab}^T\E{f}_{ab}\leq\frac{\gamma}
{\sum_{j=1}^{V(\E{C}_a)}(\E{n}_{ab}^T\E{v}_a^j(\theta)-d_{ab})+
\sum_{j=1}^{V(\E{C}_b)}(d_{ab}-\E{n}_{ab}^T\E{v}_b^j(\theta))}.
\end{align*}
\end{small}

\subsection{Tunneling-Free, Second-Order Convergent Grasp Planner}
We present our complete formulation below:
\begin{tiny}
\begin{align}
\label{eq:SO}
\argmax{\AAA{\theta,\E{n}_{ab},d_{ab}},\BBB{Q,\E{f}_{ab}}}&
\sum_{\substack{a=1,\cdots,M\\b=M+1,\cdots,M+N}}
\gamma\sum_{j=1}^{V(\E{C}_a)}\E{log}(\AAA{\E{n}_{ab}^T\E{v}_a^j(\theta)}-\AAA{d_{ab}})  \\
&+\sum_{\substack{a=1,\cdots,M\\b=M+1,\cdots,M+N}}
\gamma\sum_{j=1}^{V(\E{C}_b)}\E{log}(\AAA{d_{ab}}-\AAA{\E{n}_{ab}^T\E{v}_b^j(\theta)})+\BBB{Q}\nonumber \\
\ST&\BBB{Q}\leq \sum_j{\E{s}^d}^T\BBB{\E{f}_{ab}}\quad\forall  ab\nonumber   \\
&\AAA{\E{n}_{ab}^T}\BBB{\E{f}_{ab}}\leq\frac{\gamma}
{\sum_{j=1}^{V(\E{C}_a)}(\AAA{\E{n}_{ab}^T\E{v}_a^j(\theta)}-\AAA{d_{ab}})+
\sum_{j=1}^{V(\E{C}_b)}(\AAA{d_{ab}}-\AAA{\E{n}_{ab}^T\E{v}_b^j(\theta)})}\nonumber \\
&\mu\AAA{\E{n}_{ab}^T}\BBB{\E{f}_{ab}}\geq\|\left(\E{I}-\AAA{\E{n}_{ab}\E{n}_{ab}^T}\right)\BBB{\E{f}_{ab}}\|.\nonumber
\end{align}
\end{tiny}
This optimization will be solved using ADMM, note that when we fix $\theta,\E{n}_{ab},d_{ab}$ and optimize $Q,\E{f}_d^j$ the problem is convex. Otherwise, the problem is non-convex, non-linear. This algorithm is outlined in \prettyref{alg:second_order}.
\begin{algorithm}[ht]
\caption{Solve \prettyref{eq:SO} \CMT{(Work ongoing)}.}
\label{alg:second_order}
\begin{algorithmic}[1]
\Require{Initial guess $\E{n}_{ab}^0,d_{ab}^0,\theta^0$.}
\For{Iteration $k=0,\cdots$}
\LineComment{Convex solver e.g. Mosek}
\State{Solve Eq\ref{eq:SO} (given $\E{n}_{ab}^k,d_{ab}^k,\theta^k$) for $Q^k,\left[\E{f}_d^i\right]^k$}
\LineComment{Non-convex, Newton-type, primal-only solver}
\State{Solve Eq\ref{eq:SO} (given $Q^k,\left[\E{f}_d^i\right]^k$) for $\E{n}_{ab}^{k+1},d_{ab}^{k+1},\theta^{k+1}$}
\If{$|Q^{k+1}-Q^k|<\epsilon$}
\State Return $Q^k,\left[\E{f}_d^i\right]^k,\E{n}_{ab}^{k+1},d_{ab}^{k+1},\theta^{k+1}$
\EndIf
\EndFor

\end{algorithmic}
\end{algorithm}
